Equivariant Transformer Networks

How can prior knowledge on the transformation invariances of a domain be incorporated into the architecture of a neural network? We propose Equivariant Transformers (ETs), a family of differentiable image-to-image mappings that improve the robustness of models towards pre-defined continuous transformation groups. Through the use of specially-derived canonical coordinate systems, ETs incorporate functions that are equivariant by construction with respect to these transformations. We show empirically that ETs can be flexibly composed to improve model robustness towards more complicated transformation groups in several parameters. On a real-world image classification task, ETs improve the sample efficiency of ResNet classifiers, achieving relative improvements in error rate of up to 15% in the limited data regime while increasing model parameter count by less than 1%.

==> background.tex <==
\section{Background}
\label{sec:background}


==> introduction-old.tex <==
\section{Introduction}
\label{sec:introduction}

% something everyone agrees with
% core motivation: invariance to pose
%An object's appearance in a scene is a function not only of its type, but also of its pose relative to the observer.
%For example, variations in pose can manifest as differences in position, rotation, scale, and perspective in an image.
The appearance of an object in an image 
Achieving invariance to variations in object pose is a central challenge in image classification, object detection, face recognition, and many other tasks in computer vision~\citep{Mundy1992}.

% something problematic
Realizing pose invariance in practice is a challenging problem since small changes in pose can result in large pixel-level differences in object appearance.
For current methods based on convolutional neural networks (CNNs), this variability translates to reduced statistical and computational efficiency.
From a statistical perspective, the need to learn distinct convolutional filters sensitive to the appearance of an object in each pose results in poor sample complexity in training.
Computationally, the evaluation of large filter banks in each layer of the network is costly at both training and inference time.
%Indeed, state-of-the-art CNN-based image classifiers have recently been shown to lack robustness to small affine transformations of input images \citep{engstrom2017rotation,kanbak2018geometric}.

% canonicalization
These issues can be mitigated if it were possible to reverse the effect of nuisance pose parameters, thereby obtaining \emph{canonicalized} views of objects prior to subsequent operations such as classification.
This canonicalize-then-classify approach underpins previous work on Spatial Transformer (ST) networks \citep{jaderberg2015spatial}, which attempt to canonicalize object appearance by predicting inverse transformations conditioned on the input image.
However, the pose prediction component of STs is itself typically parameterized as a CNN, leading to similar sample efficiency issues as with regular CNNs~\citep{esteves2018polar}.

% what we do in this paper
% *compositions* of transformations distinguish from other recent work on equivariance
We propose the use of \emph{Equivariant Transformers}~(ETs), a family of functions that incorporates equivariance with respect to target transformations such as rotation, shear, and perspective.
As with standard ST layers, ETs can be used as drop-in ``pre-filters'' that canonicalize an input image before subsequent processing.
In contrast with ST layers, ETs use pose prediction functions that guarantee \emph{self-consistent} outputs: for example, if an input image is rotated by an angle $\theta$, then the predicted rotation will likewise be incremented by $\theta$.
Self-consistent pose predictors therefore ensure that an entire set of images on the orbit of a transformation is mapped to the same canonical form. 
%In this paper, we propose an extension of the Spatial Transformer that achieves improved data efficiency and geometric robustness.
%These improvements stem from the incorporation of prior knowledge on the types of transformations that have been applied to input images.
%Unlike standard STs, we ensure that pose parameters are predicted using functions that are \emph{equivariant} with respect to the specified transformations.
%The equivariance condition that we impose on the pose prediction functions ensures \emph{self-consistency}---for example, if an input image is rotated by an angle $\theta$, then the predicted rotation will likewise be incremented by $\theta$.

% what's challenging/technical contribution
The resulting challenge is to design a class of functions that achieves this self-consistency property.
We demonstrate that self-consistent pose predictors can be constructed for any smooth, invertible, one-parameter family of transformations in the image plane.
The key idea is to use the method of \emph{canonical coordinates} for Lie transformation groups~\citep{rubinstein1991recognition}:
this technique allows us to guarantee equivariance in a computationally efficient manner without requiring sample-inefficient heuristics such as data augmentation.
For several-parameter transformations such as affine and projective maps, we can apply a sequence of ET layers, each tailored to a particular one-parameter subgroup of the full transformation group (\emph{e.g.}, rotation, or translation along a given axis).
%For practitioners, this formulation allows for easy experimentation with multiple combinations of transformation types.

% experiments
Empirically, we show that ETs improve the accuracy of CNNs on image classification tasks where objects are distorted by changes in the relative position of the observer.
%On an MNIST variant where the digits are distorted by projective deformations such as rotation, scale, skew, and perspective transformations. 
For example, on the Street View House Numbers (SVHN) dataset, we show that ET layers improve the sample efficiency of ResNet classifiers: in the limited data regime, we observe relative improvements in error rate of up to $15\%$.

\iffalse
A longstanding challenge in computer vision is the design of object recognition systems 
that are invariant to geometric transformations \citep{khotanzad1990classification,wood1996invariant,lowe2004distinctive}.
While standard convolutional neural networks (CNNs) achieve invariance to translations through 
a combination of spatial convolutional layers and pooling, there is no similar invariance guarantee for other families of transformations such as rotation, scaling, and shifts in perspective \citep{engstrom2017rotation,kanbak2018geometric}.
Typical efforts to improve the geometric robustness of CNNs are costly both during training and inference.
For instance, data augmentation increases training time due to the need to synthesize and process perturbed versions of 
training examples, while the incorporation of convolutional filters sensitive to different
poses results in both increased memory usage and computational cost at inference time.

In this paper, we propose a method for learning image classifiers with improved invariance properties
with respect to geometric transformations of the input. 
In the vein of Spatial Transformer Networks (STNs) \citep{jaderberg2015spatial}, our proposed architecture separates
the classifier into two components: a \emph{canonicalization} component that returns a transformed view of an
input image, and a \emph{classification} component that receives the canonicalized image and outputs the prediction.
The goal of this two-stage pipeline is to factorize the \emph{geometric robustness} and \emph{template matching} capabilities of the classifier, with the hypothesis that such a factorization allows for a simpler representation of the classifier as a whole.

Our primary contribution is an iterative canonicalization process with \emph{equivariant} prediction of pose parameters at each stage: that is, a transformation of the input with parameter $\phi$ will yield a pose prediction incremented by $\phi$.
As a motivating example, consider an image $x$ that has been transformed by a rotation $R_\theta$ and translation $T_t$ with unknown parameters $\theta\in\R$ and $t\in\R^2$, such that $\tilde{x} = T_{t}(R_\theta(x))$. % TODO: move this example down
Given $\tilde{x}$, our goal is to recover the original image $x$.
In a standard STN, the pose parameters $(\theta, t)$ are directly predicted using a CNN that takes $\tilde{x}$ as input.
The problem here is that standard CNNs lack rotational equivariance---consequently, the STN pose prediction may be unstable with respect to small rotational perturbations of the input, and there is no guarantee of generalization to pose parameters not seen at training time.
In contrast, we predict the pose parameters $(\theta, t)$ using a two stage procedure: 
we first predict the shift $\hat{t}$ from $\tilde{x}$ using a standard CNN, and then predict the angle $\hat{\theta}$ from $T_{-\hat{t}}(\tilde{x}) \approx R_\theta(x)$ using a \emph{rotationally equivariant} network.
 More generally, this inversion process can be further iterated to handle more deeply nested compositions of transformations. For transformations other than rotation, we employ pose prediction networks that are equivariant to the particular transformation.

We achieve equivariant pose prediction with respect to continuous transformation groups through the use of specially constructed \emph{canonical coordinates} \citep{rubinstein1991recognition}. 
Under the appropriate canonical coordinate system, a deformation of the input image by a transformation with parameter $\phi$ becomes a corresponding translation by $\phi$.
We can therefore reduce the problem of group-equivariant pose prediction to that of \emph{translation}-equivariant pose prediction using a CNN.
Due to the link between our method and the long line of previous work on \emph{image registration} under geometric transformations \citep{de1987registration,reddy1996fft,derrode2001robust}, we refer to our proposed architecture as a Geometric Registration Network (GRN).

Our empirical results...
MNIST...
Adapting pre-trained networks...

The rest of the paper proceeds as follows. We first review related work (Sec.~\ref{sec:related}), ... relevant background on (Sec.~\ref{sec:background}) (Sec.~\ref{sec:method}) empirical evaluation (Sec.~\ref{sec:experiments}), and we conclude with a discussion of  (Sec.~\ref{sec:discussion})
\fi

